DivideMix: Learning with Noisy Labels as Semi-supervised Learning

Deep neural networks are known to be annotation-hungry. Numerous efforts have been devoted to reducing the annotation cost when learning with deep networks. Two prominent directions include learning with noisy labels and semi-supervised learning by exploiting unlabeled data. In this work, we propose DivideMix, a novel framework for learning with noisy labels by leveraging semi-supervised learning techniques. In particular, DivideMix models the per-sample loss distribution with a mixture model to dynamically divide the training data into a labeled set with clean samples and an unlabeled set with noisy samples, and trains the model on both the labeled and unlabeled data in a semi-supervised manner. To avoid confirmation bias, we simultaneously train two diverged networks where each network uses the dataset division from the other network. During the semi-supervised training phase, we improve the MixMatch strategy by performing label co-refinement and label co-guessing on labeled and unlabeled samples, respectively. Experiments on multiple benchmark datasets demonstrate substantial improvements over state-of-the-art methods. Code is available at https://github.com/LiJunnan1992/DivideMix .

==> cifar.tex <==
\begin{table}[!t]
	\centering
	\caption
		{
		%\small	
			Validation accuracy on CIFAR-10 and CIFAR-100.
		}
	\label{tbl:ensemble}
	%\resizebox{\textwidth}{!}{
	\begin{tabular}{l l |c|c|c|c} 
		\toprule	 	
			Methods/Noise ratio & & 20\% & 50\%& 80\% & 90\% \\
			\midrule
			\multirow{2}{*}{CE} & Best &  86.8 &  79.4& & \\
			&Last&82.7& 57.9& & \\
			\midrule
			\multirow{2}{*}{Bootstrap}~\cite{} & Best &  86.8&79.8 & & \\
			&Last&82.9& 58.4& & \\
			\midrule
			\multirow{2}{*}{Forward} & Best &  86.8 &79.8 & & \\
			&Last&83.1&59.4 & & \\
			\midrule
			\multirow{2}{*}{Mixup}~\cite{} & Best &  95.6&87.1 & & \\
			&Last&92.3& 77.6& & \\	
			\midrule			
			\multirow{2}{*}{Mixup-Bootstrap}~\cite{} & Best &  94.0& 92.0& & \\
			&Last&93.8&91.9 & & \\									                            
		\bottomrule
\end{tabular}
%}
\end{table}			














